Unsupervised Learning of the Set of Local Maxima

This paper describes a new form of unsupervised learning, whose input is a set of unlabeled points that are assumed to be local maxima of an unknown value function v in an unknown subset of the vector space. Two functions are learned: (i) a set indicator c, which is a binary classifier, and (ii) a comparator function h that given two nearby samples, predicts which sample has the higher value of the unknown function v. Loss terms are used to ensure that all training samples x are a local maxima of v, according to h and satisfy c(x)=1. Therefore, c and h provide training signals to each other: a point x' in the vicinity of x satisfies c(x)=-1 or is deemed by h to be lower in value than x. We present an algorithm, show an example where it is more efficient to use local maxima as an indicator function than to employ conventional classification, and derive a suitable generalization bound. Our experiments show that the method is able to outperform one-class classification algorithms in the task of anomaly detection and also provide an additional signal that is extracted in a completely unsupervised way.

==> GO.tex <==
\begin{table}[t]
\caption{GO analysis of the genes most correlated locally with $h$.}
\label{tab:cancergo}
\centering
\begin{tabular}{lp{6.4cm}cc}
\toprule
GO term	& Description	& P-value&	FDR q-value\\
\midrule
GO:0004984	& olfactory receptor activity&	2.11E-12&	9.72E-9	\\
GO:0004930	& G-protein coupled receptor activity&	7.12E-9	&1.64E-5\\
GO:0004888	&transmembrane signaling receptor activity	&4.47E-7	&6.85E-4\\
GO:0038023&	signaling receptor activity	&9.99E-7&	1.15E-3	\\
GO:0060089&	molecular transducer activity&	1.65E-6&	1.52E-3	\\
GO:0031856&	parathyroid hormone receptor binding&	6.15E-4	&4.72E-1	\\
GO:0031857&	type 1 parathyroid hormone receptor binding	& 6.15E-4&	4.04E-1	\\
\bottomrule
\end{tabular}
\caption{GO analysis of the genes most correlated locally with the first PCA.}
\label{tab:cancergo_pca}
\centering
\begin{tabular}{lp{6.4cm}cc}
\toprule
GO term	& Description	& P-value&	FDR q-value\\
\midrule
 GO:0050733&	RS domain binding	&2.16E-4	&9.95E-1\\
 GO:0051015&	actin filament binding	&5.31E-4	&1\\
\bottomrule
\end{tabular}
\end{table}

%GMAIL: A link to your GOrilla results has a link but also the files (last email that day)
% GO term	Description	P-value	FDR q-value	Enrichment (N, B, n, b)	Genes
% GO:0004984	olfactory receptor activity	2.11E-12	9.72E-9	7.93 (17878,364,130,21)	[+] Show genes
% GO:0004930	G-protein coupled receptor activity	7.12E-9	1.64E-5	8.99 (17878,760,34,13)	[+] Show genes
% GO:0004888	transmembrane signaling receptor activity	4.47E-7	6.85E-4	8.61 (17878,1154,18,10)	[+] Show genes
% GO:0038023	signaling receptor activity	9.99E-7	1.15E-3	5.39 (17878,1366,34,14)	[+] Show genes
% GO:0060089	molecular transducer activity	1.65E-6	1.52E-3	5.18 (17878,1421,34,14)	[+] Show genes
% GO:0031856	parathyroid hormone receptor binding	6.15E-4	4.72E-1	1,625.27 (17878,1,11,1)	[+] Show genes
% GO:0031857	type 1 parathyroid hormone receptor binding	6.15E-4	4.04E-1	1,625.27 (17878,1,11,1)	[+] Show genes

%A link to your GOrilla results - sorted_genes3_pca.txt
% GO term	Description	P-value	FDR q-value	Enrichment (N, B, n, b)	Genes
% GO:0050733	RS domain binding	2.16E-4	9.95E-1	145.71 (17850,5,49,2)	[+] Show genes
% GO:0051015	actin filament binding	5.31E-4	1E0	97.54 (17850,183,2,2)	[+] Show genes



% 		  self.conv1 = nn.Conv2d(1, 10, kernel_size=5)
%         self.conv2 = nn.Conv2d(10, 20, kernel_size=5)
%         self.conv2_drop = nn.Dropout2d()
%         self.fc1 = nn.Linear(320, 50)
%         self.fc2 = nn.Linear(50, 10)


==> fourcolumnstreetsigns.tex <==
Next, following~\cite{pmlr-v80-ruff18a}, we evaluate our method on data from the German Traffic Sign Recognition (GTSRB) Benchmark~\cite{Houben-IJCNN-2013}. The dataset contains 43 classes, from which one class (stop signs, class \#15) was used by~\cite{pmlr-v80-ruff18a}. We employ this data in order to evaluate four one-class tasks: (i) the conventional task, in which a class is compared to images out of all other tasks; (ii) the adversarial attach task, in which images are compared to images obtained by applying an attach on a multiclass classifier; (iii) class image vs. noise image, as above, using Gaussian noise with a fixed noise level of $\sigma=0.2$; (iv) same as (iii) only that after training on one class, we evaluate on images from all classes. Note that~\cite{pmlr-v80-ruff18a} presented results only for task (ii). We were not able to obtain their data and generated data for the same Boundary Attack, using the Foolbox toolbox~\cite{foolbox} on the network obtained from~\url{https://github.com/apsdehal/traffic-signs-recognition}.

The results are presented, for the first 20 classes of GTSRB, in Tab.~\ref{tab:GTSRB}. The reported results are an average over 10 random runs. The results we obtain on class 15 for the second task for the Deep-SVDD method are almost identical to those reported by~\cite{pmlr-v80-ruff18a} (80.2 vs 80.3). Compared to $c$ and $h$, this baseline method is able to better distinguish these cases for the vast majority of the 20 classes. However, on the conventional one-class task, both our $c$ and $h$ networks outperform the baseline method, with $c$ performing better than $h$, as in the MNIST and CIFAR experiments. The two results could be linked: if $c$ happens to be more aligned with the multiclass classifier, then it would be fooled more easily by the adversarial attacks designed for that classifier. In addition, the results indicated that $h$ captures image noise better than both $c$ and Deep-SVDD.

\begin{table}[t]
\caption{Results obtained on the GTSRB dataset on four one-class tasks. Reported are AUC values in percents. DS denotes Deep-SVDD by~\cite{pmlr-v80-ruff18a}.}
\label{tab:GTSRB}
\centering
\begin{tabular}{lcccccccccccc}
\toprule
Class  & \multicolumn{3}{c}{(i) Multiclass} & \multicolumn{3}{c}{(ii) Adversarial}& \multicolumn{3}{c}{(iii) Noise in-class} & \multicolumn{3}{c}{(iv) Noise all images. }\\
  \cmidrule(l{5pt}r{5pt}){2-4}
  \cmidrule(l{5pt}r{5pt}){5-7}
  \cmidrule(l{5pt}r{5pt}){8-10}
  \cmidrule(l{5pt}r{5pt}){11-13}
 & $c$ & $h$ & DS & $c$ & $h$ & DS & $c$ & $h$ & DS & $c$ & $h$ & DS\\
\midrule
1  & 92.6 & 77.8 & 86.2 & 72.1 & 90.2 & 89.9 & 61.1 & 62.3 & 61.8 & 55.1 & 58.9 & 44.7 \\
2  & 78.0 & 75.4 & 71.9 & 55.0 & 61.2 & 75.0 & 75.6 & 96.3 & 74.7 & 71.4 & 92.3 & 51.4 \\
3  & 78.3 & 79.5 & 65.8 & 52.5 & 64.0 & 81.0 & 71.0 & 95.0 & 66.1 & 79.0 & 98.5 & 50.0 \\
4  & 79.7 & 81.7 & 63.9 & 67.1 & 61.0 & 90.0 & 89.1 & 97.0 & 66.3 & 71.0 & 82.0 & 53.2 \\
5  & 79.7 & 79.3 & 73.2 & 58.0 & 53.1 & 86.9 & 90.1 & 95.6 & 48.7 & 72.3 & 84.5 & 56.3 \\
6  & 73.8 & 66.4 & 81.8 & 71.2 & 71.9 & 83.4 & 91.1 & 85.3 & 88.1 & 75.3 & 75.2 & 62.0 \\
7  & 91.0 & 90.2 & 73.6 & 69.1 & 64.1 & 96.6 & 93.0 & 94.1 & 84.1 & 58.1 & 72.4 & 55.2 \\
8  & 82.1 & 75.4 & 74.6 & 55.0 & 63.0 & 84.1 & 93.7 & 93.9 & 51.6 & 71.0 & 82.1 & 56.7 \\
9  & 80.2 & 84.7 & 73.4 & 58.0 & 60.0 & 88.3 & 92.4 & 93.7 & 54.3 & 70.5 & 81.0 & 53.8 \\
10 & 85.8 & 74.9 & 79.2 & 61.3 & 51.4 & 88.0 & 82.0 & 93.4 & 88.7 & 71.0 & 84.0 & 57.7 \\
11 & 81.9 & 81.7 & 82.7 & 51.2 & 59.0 & 79.8 & 93.4 & 93.9 & 65.0 & 78.2 & 78.4 & 68.3 \\
12 & 86.9 & 84.6 & 54.3 & 58.0 & 60.0 & 83.0 & 78.3 & 92.6 & 89.8 & 70.3 & 89.1 & 64.5 \\
13 & 88.1 & 82.1 & 60.0 & 60.1 & 60.5 & 69.0 & 84.0 & 91.2 & 74.6 & 78.2 & 79.1 & 60.5 \\
14 & 93.5 & 93.7 & 57.6 & 64.0 & 55.0 & 83.0 & 82.3 & 85.4 & 78.9 & 76.0 & 77.4 & 63.4 \\
15 & 98.2 & 93.7 & 71.9 & 56.3 & 64.0 & 80.2 & 67.3 & 81.2 & 65.0 & 54.0 & 64.0 & 49.2 \\
16 & 87.6 & 90.5 & 71.8 & 54.0 & 65.0 & 89.8 & 59.0 & 78.3 & 90.0 & 55.3 & 63.2 & 55.6 \\
17 & 92.5 & 96.8 & 76.7 & 40.2 & 60.1 & 93.2 & 73.1 & 83.4 & 83.1 & 58.3 & 67.2 & 55.6 \\
18 & 99.3 & 85.4 & 64.4 & 55.0 & 55.1 & 72.8 & 73.0 & 92.1 & 77.7 & 87.3 & 97.2 & 50.7 \\
19 & 79.5 & 79.7 & 52.2 & 54.2 & 53.9 & 83.5 & 68.1 & 81.2 & 90.4 & 62.0 & 78.3 & 57.8 \\
20 & 92.9 & 92.9 & 52.1 & 55.2 & 65.0 & 97.5 & 76.3 & 78.2 & 81.6 & 52.3 & 63.0 & 74.0 \\
\midrule
Avg & {\bf 86.1} & 83.3 & 69.4 & 58.4 & 61.9 & {\bf 84.7} & 79.7 & {\bf 88.2} & 74.0 & 68.3 & {\bf 78.4} & 57.0\\
\bottomrule
\end{tabular}
\end{table}

